"I thought it was my mistake, but it's really the design'': A Critical Examination of the Accessibility of User-Enacted Moderation Tools on Facebook and X

As social media platforms increasingly promote the use of user-enacted moderation tools (e.g., reporting, blocking, content filters) to address online harms, it becomes crucially important that such controls are usable for everyone. We evaluate the accessibility of these moderation tools on two mainstream platforms -- Facebook and X -- through interviews and task-based walkthroughs with 15 individuals with vision impairments. Adapting the lens of \emph{administrative burden of safety work}, we identify three interleaved costs that users with vision loss incur while interacting with moderation tools: \emph{learning costs} (understanding what controls do and where they live), \emph{compliance costs} (executing multi-step procedures under screen reader and low-vision conditions), and \emph{psychological costs} (experiencing uncertainty, stress, and diminished agency). Our analysis bridges the fields of content moderation and accessibility in HCI research and contributes (1) a cross-platform catalog of accessibility and usability breakdowns affecting safety tools; and (2) design recommendations for reducing this burden.

==> acmart-preload-hook.tex <==
% Loaded by acmart *before* it loads any packages.
% Make hyperref load early to satisfy hyperxmp's requirement.
\PassOptionsToPackage{unicode,bookmarksnumbered}{hyperref}% optional but common
\RequirePackage{hyperref}
